WIN-PDQ: A Wiener-estimator-based projection-domain quantitative SPECT method that accounts for intra-regional uptake heterogeneity

SPECT can enable the quantification of activity uptake in lesions and at-risk organs in {\alpha}-particle-emitting radiopharmaceutical therapies ({\alpha}-RPTs). But this quantification is challenged by the low photon counts, complicated isotope physics, and the image-degrading effects in {\alpha}-RPT SPECT. Thus, strategies to optimize the SPECT system and protocol designs for the task of regional uptake quantification are needed. Objectively performing this task-based optimization requires a reliable (accurate and precise) regional uptake quantification method. Conventional reconstruction-based quantification (RBQ) methods have been observed to be erroneous for {\alpha}-RPT SPECT. Projection-domain quantification methods, which estimate regional uptake directly from SPECT projections, have demonstrated potential in providing reliable regional uptake estimates, but these methods assume constant uptake within the regions, an assumption that may not hold. To address these challenges, we propose WIN-PDQ, a Wiener-estimator-based projection-domain quantitative SPECT method. The method accounts for the heterogeneity within the regions of interest while estimating mean uptake. An early-stage evaluation of the method was conducted using 3D Monte Carlo-simulated SPECT of anthropomorphic phantoms with radium-223 uptake and lumpy-model-based intra-regional uptake heterogeneity. In this evaluation with phantoms of varying mean regional uptake and intra-regional uptake heterogeneity, the WIN-PDQ method yielded ensemble unbiased estimates and significantly outperformed both reconstruction-based and previously proposed projection-domain quantification methods. In conclusion, based on these preliminary findings, the proposed method is showing potential for estimating mean regional uptake in {\alpha}-RPTs and towards enabling the objective task-based optimization of SPECT system and protocol designs.

==> SPIE_Abstract_v1.tex <==
\textbf{A Wiener-estimator-based projection-domain quantitative SPECT
method: addressing intra-regional uptake heterogeneities with
kernel-based modeling}

\textbf{Zekun Li\textsuperscript{1}, Abhinav K.
Jha\textsuperscript{1,2}}

\textsuperscript{1}Department of Biomedical Engineering, Washington
University in St. Louis, St. Louis, MO, USA

\textsuperscript{2}Mallinckrodt Institute of Radiology, Washington
University in St. Louis, St. Louis, MO, USA

\textbf{Abstract}

\textbf{Description of Purpose}
Alpha-particle-emitting radiopharmaceutical therapies (α-RPTs) is
gaining increasing clinical significance {[}{]}. In these therapies,
systemically administered radiopharmaceuticals distribute throughout the
patient, accumulating to unknown levels at sites of disease and in
radiosensitive vital organs {[}{]}. Thus, it is important to quantify
the absorbed doses of the lesions and different organs of the patient
treated with these potent agents to adapt treatment regimens, predict
therapy outcomes, and monitor adverse events {[}{]}.

Often, α-particle-emitting isotopes also emit X- and γ-ray photons,
providing a mechanism to quantify the absorbed dose by measuring the
activity uptake in organs and lesions using quantitative single-photon
emission computed tomography (SPECT)-based methods. Conventional
quantitative SPECT methods usually use reconstruction-based
quantifications (RBQ). These methods first obtain reconstructed SPECT
images and volume-of-interest (VOI) definitions corresponding to lesions
and organs of the patient. Then, the regional mean activity uptake
values are obtained by averaging the voxel values within each VOI.
However, these approaches have been observed to be challenged by the
extremely low number of detected photon-counts in α-RPTs, yielding
region uptake estimates with high bias (10-35\%) and standard deviation
(12-30\%) in previous studies {[}{]}.

We recognized that the task for the quantitative SPECT in α-RPT is to
estimate the regional uptake of lesions and organs. The major challenge
with the RBQ methods is that they require an intermediate step to
estimate a large number of voxel values given the limit number of
detected counts. This step is not only ill-posed, but also subject to
information loss {[}{]}. The methods then estimate the regional uptake
based on the reconstructed voxel values, which may already been in
accurate. Additionally, averaging the voxel values within each VOI is
not an optimal approach to estimate the regional uptake, since it has
been shown that the reconstructed voxel values in SPECT follow a
log-normal distribution.

Projection-domain quantitative SPECT methods estimate the target values
directly from SPECT projections, skipping the reconstruction step. These
methods, such as the scanning-linear {[}{]}, Wiener {[}{]}, and
maximum-likelihood (ML) {[}{]} estimator-based methods, have
demonstrated significant potentials in previous studies. Especially, a
recently developed low-count quantitative SPECT (LC-QSPECT) method,
using ML estimator, has demonstrated the ability to yield precise and
accurate estimates of regional activity uptake in α-RPT SPECT, given
that the accurate VOI-definitions with homogeneous intra-regional uptake
are available {[}{]}. However, to the best of our knowledge, none of
these projection-domain quantification methods explicitly accounted for
the potential heterogenous uptake distributions within each region when
estimating the mean regional uptake values. Given the potent that, by
making use of information in CT scans and the SPECT reconstruction as
well as the information in previous scanning of the patient, we could
segment the VOIs that contain activity uptake as homogeneous as
possible, the intra-regional heterogeneous uptake could still present.
Although, the LC-QSPECT method has been observed to yield reliable
regional uptake estimates given intra-lesion uptake heterogeneities
{[}{]}, the method has been observed to be less accurate given a
significant level of heterogeneous uptake in all large regions, as we
will also show in the results to be present later.

Since the task is to estimate the mean regional uptake values, the
intra-regional uptake heterogeneities can be treated as nuisance
parameters. As shown in {[}{]}, the optimal strategy to deal with the
nuisance parameters is to marginalize over them. Given the fact that, it
is more feasible to marginalize over nuisance parameters in linear
estimator and Wiener estimator is the linear estimator that achieves the
minimum ensemble mean squared error (EMSE), in this study, we develop
and evaluate a Wiener-estimator-based projection-domain quantitative
SPECT method, that estimate the mean regional uptake directly from SPECT
projections, while marginalize the intra-regional uptake heterogeneities
(Wiener INtegration Projection-Domain Quantification method, WIN-PDQ
method). We specifically provide solutions for intra-regional uptake
heterogeneities that can be describe by certain kinds of kernel-based
models, and evaluated the method using 2D anthropomorphic phantom with
lumpy-model-based intra-regional heterogeneities {[}{]}.

\textbf{Method}

In this section, we first present the theory of the proposed WIN-PDQ method. In the theory part, we first derive the general form of the WIN-PDQ method that consider all kinds of parameterized intra-regional uptake heterogeneities; then we derive the analytical solution for the estimator, considering lumpy-based intra-regional uptake heterogeneity modeling. Next, we describe the experiments we conducted to validate and
evaluate the WIN-PDQ method.

1. Theory

1.1 General form of Wiener estimator that marginalize over
intra-regional heterogeneities

Denote the activity uptake distribution within a patient by
\(f(\mathbf{r|\theta})\), where \(\mathbf{r} = (x,y,z)\) denote the
spatial 3-D coordinates and \(\mathbf{\theta}\) denotes the parameters
that describe the intra-regional uptake heterogeneities of the patient.
Considering that there are in total \(K\) VOIs in the patient, denote
the mean regional uptake value and VOI function of the \(k^{th}\) VOI as
\(\lambda_{k}\) and \(\phi_{k}(\mathbf{r})\), respectively. We have

\[\begin{matrix}
\phi_{k}\left( \mathbf{r} \right) = \left\{ \begin{matrix}
\& 1,\ \ \ if\ \mathbf{r}\ lies\ within\ the\ k^{th}\ VOI, \\
\& 0,\ \ \ otherwise, \\
\end{matrix} \right.\ \#(1) \\
\end{matrix}\]

and

\[\begin{matrix}
\lambda_{k} = \frac{\int_{}^{}{d^{3}r\ f\left( \mathbf{r} \middle| \mathbf{\theta} \right)\phi_{k}\left( \mathbf{r} \right)}}{\int_{}^{}{d^{3}r\ \phi_{k}\left( \mathbf{r} \right)}}.\#(2) \\
\end{matrix}\]

Considering a SPECT system imaging the patient, denote the measured
projection data by \(M\)-dimensional vector \(\mathbf{g}\) and the SPECT
system by the operator \(\mathcal{H}\). Similar to that in {[}{]},
denote the stray-radiation-related noise that become significant at low
counts by \(\Psi,\) where \(\Psi\) is a \(M\)-dimensional vector with
each element equal to \(\psi\), the mean value of this noise in each
projection bin. Then, the projection data \(\mathbf{g}\) are Poisson
distributed with mean of \(\mathcal{H}\mathbf{f} + \mathbf{\Psi}\). The
imaging system equation is given by

\[\begin{matrix}
\mathbf{g} = \mathcal{\ H}\mathbf{f} + \mathbf{\Psi}\mathbf{+ n.}\mathbf{\#}(3) \\
\end{matrix}\]

%%
Denote the estimator matrix by \(\mathbf{W}\) and the estimated regional
uptake with given acquired data \(\mathbf{g}\) as
~\(\widehat{\mathbf{\lambda}}(\mathbf{g})\). Denote the estimates
averaged over all sources of randomness in \(\mathbf{g}\), including the
randomness due to the intra-regional heterogeneity described by
\(\mathbf{\theta}\), as
\(< < < \widehat{\mathbf{\lambda}}\left( \mathbf{g} \right)\mathbf{>}_{\mathbf{g|\lambda,\theta}}\mathbf{>}_{\mathbf{\theta|\lambda}}\mathbf{>}_{\mathbf{\lambda}}\),
where \(< \bullet >_{\mathbf{X}}\) denote average over the randomness
due to \(\mathbf{X}\) similar to that defined in {[}{]}. A linear
estimator that is globally unbiased requires that

\[\begin{matrix}
\widehat{\mathbf{\lambda}}\left( \mathbf{g} \right)\mathbf{=}\overline{\mathbf{\lambda}}\mathbf{+}\mathbf{W}^{t}\left( \mathbf{g -}\overline{\overline{\overline{\mathbf{g}}}} \right)\mathbf{,\#}(4) \\
\end{matrix}\]

where
~\(\overline{\overline{\overline{\mathbf{g}}}}\mathbf{=} < < < \mathbf{g}\mathbf{>}_{\mathbf{g|\lambda,\theta}}\mathbf{>}_{\mathbf{\theta|\lambda}}\mathbf{>}_{\mathbf{\lambda}}\).

The EMSE can be stated as

\[{EMSE = \  \ll < \ \left\lbrack \widehat{\mathbf{\lambda}}\left( \mathbf{g} \right)\mathbf{- \lambda} \right\rbrack^{\mathbf{t}}\left\lbrack \widehat{\mathbf{\lambda}}\left( \mathbf{g} \right)\mathbf{- \lambda} \right\rbrack\mathbf{>}_{\mathbf{g|\lambda,\theta}}\mathbf{>}_{\mathbf{\theta|\lambda}}\mathbf{>}_{\mathbf{\lambda}}
}{\mathbf{=}tr\mathbf{W}^{t}\mathbf{\ll < \ }\left\lbrack \mathbf{g -}\overline{\overline{\overline{\mathbf{g}}}} \right\rbrack\left\lbrack \mathbf{g -}\overline{\overline{\overline{\mathbf{g}}}} \right\rbrack^{t}\mathbf{>}_{\mathbf{g|\lambda,\theta}}\mathbf{>}_{\mathbf{\theta|\lambda}}\mathbf{>}_{\mathbf{\lambda}}\mathbf{W}
}{\mathbf{-}2tr\mathbf{\ll <}\left( \mathbf{\lambda -}\overline{\mathbf{\lambda}} \right)\left( \mathbf{g -}\overline{\overline{\overline{\mathbf{g}}}} \right)^{t}\mathbf{>}_{\mathbf{g|\lambda,\theta}}\mathbf{>}_{\mathbf{\theta|\lambda}}\mathbf{>}_{\mathbf{\lambda}}\mathbf{W}
}{\mathbf{+}tr\mathbf{<}\left( \mathbf{\lambda -}\overline{\mathbf{\lambda}} \right)\left( \mathbf{\lambda -}\overline{\mathbf{\lambda}} \right)^{t}\mathbf{>}_{\mathbf{\lambda}}
}\begin{matrix}
\mathbf{=}tr\mathbf{W}^{t}\mathbf{K}_{\mathbf{g}}\mathbf{W\  -}2tr\mathbf{K}_{\mathbf{\lambda g}}\mathbf{W +}tr\mathbf{K}_{\mathbf{\lambda}}，\mathbf{\#}\left. （5 \right.） \\
\end{matrix}\]

where \(tr\) denotes the trace of the matrix.
\(\mathbf{K}_{\mathbf{g}}\), \(\mathbf{K}_{\mathbf{\lambda g}}\), and
\(\mathbf{K}_{\mathbf{\lambda}}\) denote the covariance \(\mathbf{g}\),
cross covariance of \(\mathbf{\lambda}\) and \(\mathbf{g}\), and the
covariance of \(\mathbf{\lambda}\) based on the probability distribution
function (PDF), respectively, considering the randomness of
intra-regional uptake heterogeneity. To solve the \(\mathbf{W}\) that
minimize the EMSE, we take Fréechet derivative of Eq. (5) and get

\[\begin{matrix}
\frac{d}{d\mathbf{W}}EMSE = 2\mathbf{K}_{\mathbf{g}}\mathbf{W\  -}2\mathbf{K}_{\mathbf{\lambda g}}^{t}\mathbf{.}\#(6) \\
\end{matrix}\]

Letting the derivative to be zero, \(\mathbf{W}\) can be obtained by

\[\begin{matrix}
\mathbf{W =}{\mathbf{K}_{\mathbf{g}}^{\mathbf{-}1}\mathbf{K}}_{\mathbf{\lambda g}}^{t}.\mathbf{\#}(7) \\
\end{matrix}\ \]

%%
Now we derive the solutions for \(\mathbf{K}_{\mathbf{g}}\) and
\(\mathbf{K}_{\mathbf{\lambda g}}\), considering a specific
representation of the activity uptake distribution of the patient

\[\begin{matrix}
f\left( \mathbf{r} \middle| \mathbf{\theta} \right) = \ \sum_{k = 1}^{K}{\lambda_{k}\varphi_{k}\left( \mathbf{r} \middle| \mathbf{\theta}_{\mathbf{k}} \right)},\#(8) \\
\end{matrix}\]

where
\(\varphi_{k}\left( \mathbf{r} \middle| \mathbf{\theta}_{\mathbf{k}} \right)\)
denotes the normalized heterogeneous uptake distribution within the
\(k^{th}\) region, parameterized by \(\mathbf{\theta}_{\mathbf{k}}\).
For any \(\mathbf{\theta}_{\mathbf{k,}}\)
\(\varphi_{k}(\mathbf{r|}\mathbf{\theta}_{\mathbf{k}})\) satisifies
\(\int_{}^{}{d^{3}r\ \varphi_{k}(\mathbf{r|}\mathbf{\theta}_{\mathbf{k}})} = \int_{}^{}{d^{3}r\ \phi_{k}\left( \mathbf{r} \right)\varphi_{k}(\mathbf{r|}\mathbf{\theta}_{\mathbf{k}})} = \int_{}^{}{d^{3}r\ \phi_{k}\left( \mathbf{r} \right).\ }\)
Denote\textbf{~}\(\overline{\overline{\mathbf{g}}} = < < \mathbf{g}\mathbf{>}_{\mathbf{g|\lambda,\theta}}\mathbf{>}_{\mathbf{\theta|\lambda}},\)
we have

\[{\overline{\overline{\mathbf{g}}} = < \mathcal{H}\mathbf{f}\mathbf{>}_{\mathbf{\theta|\lambda}} + \mathbf{\Psi}
}\begin{matrix}
\mathbf{=}\sum_{k = 1}^{K}{\lambda_{k} < \mathcal{H}\varphi_{k}\left( \mathbf{r} \middle| \mathbf{\theta}_{\mathbf{k}} \right)}\mathbf{>}_{\mathbf{\theta|\lambda}} + \mathbf{\Psi.}\mathbf{\#}(9) \\
\end{matrix}\]

Denote\(\ H_{k} = \mathcal{H}{< \varphi}_{k}\left( \mathbf{r} \middle| \mathbf{\theta}_{\mathbf{k}} \right)\mathbf{>}_{\mathbf{\theta|\lambda}}\),
Eq. (9) can be written as

\[\begin{matrix}
\overline{\overline{\mathbf{g}}} = \sum_{k = 1}^{K}{\lambda_{k}H_{k}} = \mathbf{H\lambda.}\#(10) \\
\end{matrix}
\]

\[{\mathbf{K}_{\mathbf{\lambda g}} = < < < \left( \mathbf{\lambda -}\overline{\mathbf{\lambda}} \right)\left( \mathbf{g -}\overline{\overline{\overline{\mathbf{g}}}} \right)^{t}\mathbf{>}_{\mathbf{g|\lambda,\theta}}\mathbf{>}_{\mathbf{\theta|\lambda}}\mathbf{>}_{\mathbf{\lambda}}
}{\mathbf{= <}\left( \mathbf{\lambda -}\overline{\mathbf{\lambda}} \right)\left( \overline{\overline{\mathbf{g}}}\mathbf{-}\overline{\overline{\overline{\mathbf{g}}}} \right)^{t}\mathbf{>}_{\mathbf{\lambda}}
}\begin{matrix}
\mathbf{=}\mathbf{K}_{\mathbf{\lambda}}\mathbf{H}^{t}\mathbf{.\#}(11) \\
\end{matrix}\]

Next, we decompose \(\mathbf{K}_{\mathbf{g}}\) by

\[{\mathbf{K}_{\mathbf{g}} = < < < \ \left\lbrack \mathbf{g -}\overline{\overline{\overline{\mathbf{g}}}} \right\rbrack\left\lbrack \mathbf{g -}\overline{\overline{\overline{\mathbf{g}}}} \right\rbrack^{t}\mathbf{>}_{\mathbf{g|\lambda,\theta}}\mathbf{>}_{\mathbf{\theta|\lambda}}\mathbf{>}_{\mathbf{\lambda}}
}{\mathbf{= < < < \ }\left\lbrack \mathbf{g -}\overline{\mathbf{g}}\mathbf{+}\overline{\mathbf{g}}\mathbf{-}\overline{\overline{\mathbf{g}}}\mathbf{+}\overline{\overline{\mathbf{g}}}\mathbf{-}\overline{\overline{\overline{\mathbf{g}}}} \right\rbrack\left\lbrack \mathbf{g -}\overline{\mathbf{g}}\mathbf{+}\overline{\mathbf{g}}\mathbf{-}\overline{\overline{\mathbf{g}}}\mathbf{+}\overline{\overline{\mathbf{g}}}\mathbf{-}\overline{\overline{\overline{\mathbf{g}}}} \right\rbrack^{\mathbf{t}}\mathbf{>}_{\mathbf{g|\lambda,\theta}}\mathbf{>}_{\mathbf{\theta|\lambda}}\mathbf{>}_{\mathbf{\lambda}}
}{\mathbf{= < < < \ }\left\lbrack \mathbf{g -}\overline{\mathbf{g}} \right\rbrack\left\lbrack \mathbf{g -}\overline{\mathbf{g}} \right\rbrack^{\mathbf{t}}\mathbf{>}_{\mathbf{g|\lambda,\theta}}\mathbf{>}_{\mathbf{\theta|\lambda}}\mathbf{>}_{\mathbf{\lambda}}\mathbf{+ < < \ }\left\lbrack \overline{\mathbf{g}}\mathbf{-}\overline{\overline{\mathbf{g}}} \right\rbrack\left\lbrack \overline{\mathbf{g}}\mathbf{-}\overline{\overline{\mathbf{g}}} \right\rbrack^{\mathbf{t}}\mathbf{>}_{\mathbf{\theta|\lambda}}\mathbf{>}_{\mathbf{\lambda}}\mathbf{+ < \ }\left\lbrack \overline{\overline{\mathbf{g}}}\mathbf{-}\overline{\overline{\overline{\mathbf{g}}}} \right\rbrack\left\lbrack \overline{\overline{\mathbf{g}}}\mathbf{-}\overline{\overline{\overline{\mathbf{g}}}} \right\rbrack^{\mathbf{t}}\mathbf{>}_{\mathbf{\lambda}}
}{\mathbf{=}\mathbf{K}_{\mathbf{n}}\mathbf{+}\overline{\mathbf{K}_{\overline{\mathbf{g}}}}\mathbf{+ H}\mathbf{K}_{\mathbf{\lambda}}\mathbf{H}^{\mathbf{t}}\mathbf{.}}\]

(12)

Since the data \(\mathbf{g}\) are Poisson distribution and the elements
are independent with each other, denote a diagonal matrix with diagonal
elements given by the elements of vector ~\(\overline{\mathbf{g}}\) by
\(diag(\overline{\mathbf{g}})\), we have

\[\begin{matrix}
\mathbf{K}_{\mathbf{n}} = < < diag\left( \overline{\mathbf{g}} \right)\mathbf{>}_{\mathbf{\theta|\lambda}}\mathbf{>}_{\mathbf{\lambda}}\mathbf{=}diag\left( \overline{\overline{\overline{\mathbf{g}}}} \right) = diag(\mathbf{H}\overline{\mathbf{\lambda}}).\mathbf{\#}(13) \\
\end{matrix}\]

Derive from Eqs. (3), (8), and (9), we have

\[{\overline{\mathbf{K}_{\overline{\mathbf{g}}}}\mathbf{= \ll \ }\left\lbrack \overline{\mathbf{g}}\mathbf{-}\overline{\overline{\mathbf{g}}} \right\rbrack\left\lbrack \overline{\mathbf{g}}\mathbf{-}\overline{\overline{\mathbf{g}}} \right\rbrack^{\mathbf{t}}\mathbf{>}_{\mathbf{\theta|\lambda}}\mathbf{>}_{\mathbf{\lambda}}
}\begin{matrix}
\mathcal{= H <}\mathbf{\lambda}^{\mathbf{t}}\mathbf{\  <}\left\lbrack \mathbf{\varphi}\mathbf{-}\overline{\mathbf{\varphi}} \right\rbrack\left\lbrack \mathbf{\varphi}\mathbf{-}\overline{\mathbf{\varphi}} \right\rbrack^{\mathbf{t}}\mathbf{>}_{\mathbf{\theta}}\mathbf{\lambda >}_{\mathbf{\lambda}}\mathcal{H}^{\mathbf{t}}\mathbf{,\#}(14) \\
\end{matrix}\]

where \(\mathbf{\varphi}\) denotes a \(K\)-dimensional vector with the
\(k^{th}\) element as
\(\varphi_{k}\left( \mathbf{r} \middle| \mathbf{\theta}_{\mathbf{k}} \right)\)
and
\(\overline{\mathbf{\varphi}}\mathbf{= \  <}\mathbf{\varphi}\mathbf{>}_{\mathbf{\theta|\lambda}}\mathbf{.}\)

1.2 Analytical solutions with lumpy-model-based intra-regional uptake
heterogeneities

Next we specifically consider lumpy-model-based intra-regional uptake
heterogeneities and derive explicit solutions to
\(\mathbf{K}_{\mathbf{g}}\) and \(\mathbf{K}_{\mathbf{\lambda g}}\). The
lumpy model was developed by Rolland and Barret {[}{]} and has been
observed to have the ability to realistically synthesizing object of
biological tissues. The lumpy-model-based intra-regional uptake
heterogeneities are created by summing a random number of lump functions
placed randomly in the VOI. Typically, the lumpy functions are Gaussian,
but other lump profiles could be also used. In this study we consider
normalized lumpy model. Denote the lump function by
\(\Lambda( \bullet )\), mathematically,

\[\begin{matrix}
\varphi_{k}\left( \mathbf{r} \middle| \mathbf{\theta}_{\mathbf{k}} \right) = \phi_{k}\left( \mathbf{r} \right)\frac{A_{k}}{N_{k} + 1}\sum_{n = 1}^{N_{k} + 1}\frac{\Lambda\left( \mathbf{r -}\mathbf{c}_{\mathbf{n}}^{\mathbf{k}} \right|\ s_{k})}{\int_{}^{}{d\mathbf{r}^{'}}\Lambda\left( \mathbf{r}^{\mathbf{'}}\mathbf{-}\mathbf{c}_{\mathbf{n}}^{\mathbf{k}} \right|\ s_{k})\phi_{k}\left( \mathbf{r}^{\mathbf{'}} \right)},\#(15) \\
\end{matrix}\]

where
\(A_{k}\)=\(\int_{}^{}{d^{3}r\ \phi_{k}\left( \mathbf{r} \right)}\) and
\(\Lambda\) and
\(\theta_{k} = \{ N_{k},\mathbf{c}^{\mathbf{k}},s_{k}\}\). In this
function, \(N_{k},\mathbf{c}^{\mathbf{k}},and\ s_{k}\) denote the number
of lumps, the lump center locations, and the size of the lumps in the
\(k^{th}\) VOI, respectively.

We model \(s_{k}\) as a constant factor each region, \(N_{k}\) to be
Poisson distributed with mean of ~\(\overline{N_{k}}\), and the
\(n^{th}\) element of \(\mathbf{c}^{\mathbf{k}}\)\textbf{,}
\(\mathbf{c}_{\mathbf{n}}^{\mathbf{k}}\)\textbf{,} to be uniformly
distributed within the \(k^{th}\) VOI. Then,

\[{{\overline{\varphi}}_{k} = {< \varphi}_{k}\left( \mathbf{r} \middle| \mathbf{\theta}_{\mathbf{k}} \right)\mathbf{>}_{\mathbf{\theta|\lambda}}
}{= {\ \phi}_{k}\left( \mathbf{r} \right)\sum_{N_{k}}^{}{\Pr\left( N_{k} \right)\ \frac{A_{k}}{N_{k} + 1}\sum_{n = 1}^{N_{k} + 1}{\int_{}^{}{d\mathbf{c}_{\mathbf{n}}^{\mathbf{k}}}\ \frac{\Lambda\left( \mathbf{r -}\mathbf{c}_{\mathbf{n}}^{\mathbf{k}} \right|\ s_{k})}{\int_{}^{}{d\mathbf{r}^{'}}\Lambda\left( \mathbf{r}^{\mathbf{'}}\mathbf{-}\mathbf{c}_{\mathbf{n}}^{\mathbf{k}} \right|\ s_{k})\phi_{k}\left( \mathbf{r}^{\mathbf{'}} \right)}}\Pr\left( \mathbf{c}_{\mathbf{n}}^{\mathbf{k}} \right)}
}{= \int_{}^{}{d\mathbf{c}_{\mathbf{n}}^{\mathbf{k}}}\ \frac{\Lambda_{k}\left( \mathbf{r} - \mathbf{c}_{\mathbf{n}}^{\mathbf{k}} \right)}{\left( \Lambda_{k}*\phi_{k} \right)\left( \mathbf{c}_{\mathbf{n}}^{\mathbf{k}} \right)}\phi_{k}\left( \mathbf{c}_{\mathbf{n}}^{\mathbf{k}} \right)
}{= \Lambda_{k}*\frac{\phi_{k}}{\Lambda_{k}*\phi_{k}}\left( \mathbf{r} \right).}\]

(16)

Denote
\(\mathbf{K}^{\mathbf{\varphi}} = \mathbf{<}\left\lbrack \mathbf{\varphi}\mathbf{-}\overline{\mathbf{\varphi}} \right\rbrack\left\lbrack \mathbf{\varphi}\mathbf{-}\overline{\mathbf{\varphi}} \right\rbrack^{\mathbf{t}}\mathbf{>}_{\mathbf{\theta}}\)\textbf{.}
It can be easily shown that
\(\mathbf{K}_{i,j}^{\mathbf{\varphi}} = 0,\ \forall\ i \neq j.\) Then,
consider Eqs. (15) and (16), we have

\[K_{k,k}^{\mathbf{\varphi}}\left( \mathbf{r,}\mathbf{r}^{'} \right){= \phi}_{k}\left( \mathbf{r} \right)\ \phi_{k}\left( \mathbf{r}^{\mathbf{'}} \right)\ \sum_{N_{k}}^{}{\Pr{\left( N_{k} \right) \times \ }}\lbrack - \frac{1}{N_{k} + 1}{(\ \Lambda}_{k}*\frac{\phi_{k}}{\Lambda_{k}*\phi_{k}})\left( \mathbf{r} \right)\mathbf{\ }{(\Lambda}_{k}*\frac{\phi_{k}}{\Lambda_{k}*\phi_{k}})(\mathbf{r}') + \frac{A_{k}}{N_{k} + 1}\int d\mathbf{c}_{\mathbf{n}^{\mathbf{''}}}^{\mathbf{k}}\mathbf{\ }\phi_{k}\left( \mathbf{c}_{\mathbf{n}^{\mathbf{''}}}^{\mathbf{k}} \right)\frac{\Lambda_{k}\left( \mathbf{r} - \mathbf{c}_{\mathbf{n}^{\mathbf{''}}}^{\mathbf{k}} \right)}{\left( \Lambda_{k}*\phi_{k} \right)\left( \mathbf{c}_{\mathbf{n}^{\mathbf{''}}}^{\mathbf{k}} \right)}\frac{\Lambda_{k}\left( \mathbf{r}^{\mathbf{'}} - \mathbf{c}_{\mathbf{n}^{\mathbf{''}}}^{\mathbf{k}} \right)}{\left( \Lambda_{k}*\phi_{k} \right)\left( \mathbf{c}_{\mathbf{n}^{\mathbf{''}}}^{\mathbf{k}} \right)}.\#(17)\]

For a given
\(\mathbf{r' \in}{\{\phi}_{k}\left( \mathbf{r}^{\mathbf{'}} \right) = 1\}\),
we have

\[{K_{k,k}^{\mathbf{\varphi}}\left( \mathbf{r,}\mathbf{r}^{'} \right) = \phi}_{k}\left( \mathbf{r} \right)\frac{\left( 1 - e^{- \overline{N}} \right)}{\overline{N}}\lbrack - {(\ \Lambda}_{k}*\frac{\phi_{k}}{\Lambda_{k}*\phi_{k}})\left( \mathbf{r} \right)\mathbf{\ }{(\Lambda}_{k}*\frac{\phi_{k}}{\Lambda_{k}*\phi_{k}})(\mathbf{r}') + A_{k}{(\ \Lambda}_{k}*\frac{\phi_{k} \times {\ \Lambda}_{k}^{- \mathbf{r}^{\mathbf{'}}}}{\Lambda_{k}*\phi_{k} \times \Lambda_{k}*\phi_{k}})(\mathbf{r})\rbrack.\#(18)\]

2. Evaluations

2.1 Phantom design

In this study, we specifically considered patients with bone metastatic
castrate-resistant prostate cancer (bmCRPC) treated with
\textsuperscript{223}Ra-based α-RPT, the first α-RPT approved by the US
FDA. For the consideration of computational issues, in this study, we
evaluate the WIN-PDQ method using 2D anthropomorphic phantoms. To
generate anthropomorphic phantom with realistic geometry, we fist
generated VOI and attenuation maps using XCAT phantom. Then, based on
the VOI map, we generated multiple realization of intra-regional uptake
heterogeneities using lumpy model.

As shown in Fig. 1 (a-b), we considered a transverse slice of a typical
patient, with heigh and weight equal to the \(50^{th}\) percental of
U.S. male. In this transvers slice, we considered five VOIs with
potential major uptake {[}{]}, the bone, kidney, large intestine (LI),
small intestine (SI), and a lesion located in the vertebrae bone. The
rest of the region in the patient usually have similar and low uptake,
we considered those regions in another one VOI, named background (BKGD).
To simulate continuous activity distribution, the VOI and attenuation
maps had a pixel side length of 2.209 mm, with dimension of 144
\(\times\) 144, which contains the entire phantom. The 2D slice had a
thickness of 4.418 mm.

In this study, we specifically consider a lumpy model with Gaussian
lumps functions. Based on the generated VOI maps, we generated 5,000
realizations of 2D phantoms with various intra-regional uptake
heterogeneities. Across the 5,000 phantom realizations, the lump
standard deviations \(s_{k}\), was set as constant for each VOI,
obtained by \(s_{k} = \sqrt{A_{k}/(50\pi)}\). For each phantom
realization, we sample the number of lumps in each region
\(N_{k}\ \)individually from a Poisson distribution with mean of
~\(\overline{N_{k}} = 50.\) The center of each lump function
\(\mathbf{c}_{\mathbf{n}}^{\mathbf{k}}\) was also uniformly sampled from
the locations within the corresponding region. The regional uptake
values of each phantom realization were sampled from Gaussian
distributions as shown in Table 1, assuming the regional uptake values
are independent from each other. The mean regional uptake values were
selected to ensure that, in the 2D scenario, the Fisher information in
the detected SPECT projection for the mean regional uptake is similar to
that in the clinical scenario {[}{]}. Activity maps of two typical
phantom realizations are shown in Fig. 1 (c-d).

2.2 Modeling the SPECT system

In this study, we considered a dual-head GE Optima 640 SPECT system with
a high energy general purpose (HEGP) collimator. The SPECT system was
simulated using SIMIND, a well validated Monte Carlo simulation software
{[}{]}. Detailed parameters for simulating this system can be found in
{[}{]}, where we have also validated our simulation of this system
imaging \textsuperscript{223}Ra. In this study, the projections were
acquired at 60 angular positions spaced uniformly over 360°. The
projections were only acquired at a 2D slice at each angular position
with 128 projection bins, with bin side-length of 4.418 mm. Each phantom
was simulated to be imaged by 30 minutes. The photopeak window was set
as 85 keV ± 20\% {[}41{]}. The isotope emission and all relevant
image-degrading processes in SPECT were simulated. The mean of the
stray-radiation-related noise in each projection bin, \(\psi\), was
determined as described in {[}{]}, with value of 0.18. The value of this
noise in each projection bin was sample from Poisson distributions.

Implementing the WIN-PDQ method requires the system operator
\(\mathcal{H}\). We implement by discretize this operator into high
resolution pixels in the object domain. We generate projections of


2.3 Validation of the WIN-PDQ

2.4 Compared methods

2.5 Figures of merit

\textbf{Results}

\textbf{Conclusion}

\textbf{New work to be presented}

\textbf{This work has not been submitted for publication elsewhere}

\textbf{References}


==> drafts.tex <==
In this context, we recognize that voxel-based image reconstruction serves merely as an intermediary step towards estimating regional uptake, and notably, the number of VOIs requiring uptake estimation is significantly less than the total number of voxels. Thus, direct quantification of mean uptake in VOIs from projection data is a less ill-posed problem and it could avoid the information loss inherent to the reconstruction process.

Given the above considerations, projection-domain quantitative SPECT methods, which estimate target values directly from SPECT projections—including scanning-linear~\cite{whitaker2008estimating,konik2015comparison}, Wiener~\cite{barrett2013foundations,barrett2008adaptive,lin2018task}, and maximum-likelihood (ML) estimator-based approaches~\cite{carson1986maximum,li2022projection}—have shown potential in prior research. Notably, a low-count quantitative SPECT (LC-QSPECT) approach using ML estimation~\cite{li2022projection} has been developed for direct activity uptake estimation in VOIs from \(\alpha\)-RPT SPECT projections. This method can effectively compensate for the complicated SPECT physics in \(\alpha\)-RPTs and address the stray-radiation-related noise that becomes significant at low counts. The method has been observed to deliver precise and accurate regional activity uptake estimates in \(\alpha\)-RPTs, given accurately defined VOIs with uniform intra-regional uptake.

However, these projection-domain quantification techniques have not yet fully addressed the challenge of heterogeneous uptake distributions within VOIs. Studies have identified substantial heterogeneity in activity uptake within patient regions undergoing \(\alpha\)-RPT, particularly in lesions~\cite{phelps2021sodium,peng2022blind}. Overlooking such intra-regional heterogeneity can result in inaccurate uptake estimates. Consequently, there exists a crucial need for a methodology capable of estimating mean regional uptake from projection data while effectively managing the complexities of intra-regional uptake heterogeneity.

